Breaking the Unit Throughput Barrier in Distributed Systems

A multi-level random power transmit strategy that is used in conjunction with a random access protocol (RAP) (e.g. ALOHA, IRSA) is proposed to fundamentally increase the throughput in a distributed communication network. A SIR model is considered, where a packet is decodable as long as its SIR is above a certain threshold. In a slot chosen for transmission by a RAP, a packet is transmitted with power level chosen according to a distribution, such that multiple packets sent by different nodes can be decoded at the receiver in a single slot, by ensuring that their SIRs are above the threshold with successive interference cancelation. Since the network is distributed this is a challenging task, and we provide structural results that aid in finding the achievable throughputs, together with upper bounds on the maximum throughput possible. The achievable throughput and the upper bounds are shown to be close with the help of comprehensive simulations. The main takeaway is that the throughput of more than 1 is possible in a distributed network, by using a judicious choice of power level distribution in conjuction with a RAP.

==> arXiv Submission/IntroPowerCSA.tex <==
\section{Introduction}
Random access protocols (RAPs) are widely used in communication networks because of their simple distributed implementation and reasonable throughput guarantees. A particular example is the slotted ALOHA protocol that dates back to \cite{abramson1970aloha}, but is still operational for initial access acquisition in cellular, satellite, and ad hoc networks \cite{roberts1975aloha, raychaudhuri1988channel, etsi2005digital}. Some initial advances to the basic ALOHA protocol were made in \cite{choudhury1983diversity, casini2007contention,del2009high}. The basic advantage of a RAP is that it completely avoids the need of network knowledge at each node, e.g. the total number of nodes etc., and works without any coordination overhead, that can grow exponentially with the number of nodes in the network. 

The flip side of this uncoordinated communication paradigm is that packets sent simultaneously by different nodes collide, making them undecodable at the receiver node, prompting retransmissions. Thus, an important performance metric with random access is the {\it throughput} that counts the average number of packets successfully received per time slot. For the basic vanilla version of the slotted ALOHA protocol, the throughput approaches $1/e$ as the number of nodes in the network grow to infinity. Thus, the overall slot occupancy is a constant even with no coordination among nodes. 

%There is a large body of work \cite{liva, stefanovic2017asymptotic, lazaro2017finite, i2018finite, sun2017coded, capture_fading, csa_paper, 4036333, 6155698, polyanskiy2017perspective, narayanan2012iterative, sun2017coded, khaleghi2017near}, , where primary recourse is to employ advanced signal processing. e.g., 
%successive interference cancellation (SIC) at the receiver.  Another technique is called ZigZag that exploits the natural random delay seen by each nodes' transmission \cite{gollakota2008zigzag}. A good survey on modern random access protocols can be found in \cite{berioli2016modern}.
  
  

The basic idea in most of the prior work that has addressed the question of improving the throughput of RAPs \cite{liva, stefanovic2017asymptotic, lazaro2017finite, i2018finite, sun2017coded, capture_fading, csa_paper, 4036333, 6155698, polyanskiy2017perspective, narayanan2012iterative, sun2017coded, khaleghi2017near}  is to introduce redundancy in time. In particular, each node transmits its packet in multiple slots (repetition), and packets received in collision free slots are decoded first. 
The contribution of the decoded packets is then removed from slots where collision occurs (using SIC), and all packets which are now collision free are decoded. This process is recursively continued till no slots can become collision free. This process increases the throughput fundamentally. Exploiting the random delay  with ZigZag \cite{gollakota2008zigzag}, decreases the need for repetition.

This idea of using repetition code at the transmit side and employing SIC  at
the receiver end was formalized in \cite{liva}, which called it the irregular
repetition slotted ALOHA (IRSA), where the packet repetition rate is chosen
systematically and shown to achieve a throughput close to $0.97$.
A natural extension to the IRSA was to include non-trivial forward error correction codes in contrast to just using the repetition code, which is termed as coded slotted ALOHA (CSA) \cite{csa_paper}. Using a judicious choice of codes, throughput larger than IRSA is achievable as expected, with also some analytical tractability via the iterated decoding framework typically used for LDPC codes. There is a large body of follow-up work  \cite{sun2017coded, lazaro2017finite, dovelos2017finite,  i2018finite, stefanovic2017asymptotic, narayanan2012iterative}
 to \cite{liva, csa_paper}.

Even though prior work has exploited the SIC ability intelligently, one feature that it has neglected is that if the colliding packets have different power levels, some of them can still be decodable simultaneously, without the need of decoding one of the colliding packets using some other slot. Essentially, if two packets $i,j$ with received power $P_i, P_j$ collide/overlap in the same slot, then the 
$i^{th}$ ($j^{th}$) packet is decodable as long as  the  
signal to interference ratio $SIR_i = \frac{P_i}{P_j} > \beta$ ($SIR_j = \frac{P_j}{P_i} > \beta$), where $\beta > 1$ is typically fixed threshold. 
Thus, by ensuring that the power profile of colliding packets in a slot is as different as possible, simultaneous decoding of more than $1$ packet is possible, {\bf potentially achieving a throughput of more than $1$}. Since the network in distributed, and each node has to make an autonomous decision, ensuring such received power profile is non-trivial.

In this paper, we propose a random access protocol, where nodes choose which slots to use for packet transmission similar to the slotted ALOHA, or IRSA, or CSA protocol, but employ different (random) power levels (following a distribution) for transmitting packets in slots chosen for transmission. 
For example, a node can choose between two different power levels $\{H,L\}, H>L$ to transmit. Ideally, the goal of the strategy is to ensure that in any slot, both the number of packets with power level $H$, and the number of packets with power level $L$, is roughly $1$. Since $\beta>1$, first we can decode the packet with power level $H$, and subsequently the packet with power level $L$ without needing any help from other slots. Essentially, with this protocol, a slot can potentially carry more than $1$ successfully decodable packet. We call this phenomena {\it power multiplexing}. The objective is non-trivial since the network is distributed, and each node makes it transmission decisions autonomously.
In general, the protocol can choose between $n$ different power levels for transmission in any slot with random distribution $\Delta$, to exploit as much of this power multiplexing as much as possible, together with the random slot occupancy distribution ($\Lambda$) driven by a RAP, e.g., slotted ALOHA, IRSA, CSA, and the problem is to 
 optimize the throughout over $\Delta$ and $\Lambda$. 
%\begin{jointly}
% 
%\end{jointly}
\vspace{-0.2in}
\subsection{How Multi-Level Power Transmission Leads to Fundamental Gain in Throughput}
Before presenting our main results, we illustrate how introducing multiple power levels fundamentally changes the throughput for 
any RAP.  Consider the toy examples presented in Fig. 
\ref{fig:irsa_slots_rep} and Fig. \ref{fig:irsa_pc_slots_rep}. Fig. 
\ref{fig:irsa_slots_rep} represents the case of IRSA, where one user transmits in
all the four slots, and the other two users transmit in two slots, all users with identical power $P=1$. 
Performing
SIC decoding process, in the first
iteration, only packet corresponding to user $1$ is decodable. However, in
the second iteration, the decoding process gets stuck due to the collision of
packets of user $2$ and $3$, and therefore the decoding process terminates. Hence we
are only able to successfully decode one packet over four slots resulting in a
throughput of $T = 0.25$. Meanwhile, in Fig. \ref{fig:irsa_pc_slots_rep}, employing 
two power levels $P\in \{1, 4\}$ uniformly randomly in
conjunction with IRSA, in the second iteration,  the packet
corresponding to user 2 can also be decoded because its SIR is above the threshold $\beta$. Therefore, the SIC/peeling
decoder which got stuck in the second iteration in case $1$, kickstarts
again enabled by the decoding of packet of user 2, and all the three packets belonging to the three users are decoded. 
Thus, by incurring a higher average transmit power, throughput of $T = 0.75$, thrice of what we had in the first
case with no power control, is achievable. 

What is important to note is that the increase in throughput by introducing random power levels is not additive or linear, but {\bf bootstraps the ability of the SIC process to unravel many more colliding packets}.
In Fig. \ref{fig:intro_comparison}, we present simulation results, where
SA represents slotted ALOHA, while IRSA and CSA with just two power levels are denoted as 
IRSA-DPC and CSA-DPC, respectively. It is clearly evident that there is a fundamental increase in the throughput that the proposed strategy provides over and above the slotted ALOHA (denoted as SA), or IRSA or CSA, and that too using only two power levels.

The remarkable feature is that introducing just two power levels that are used randomly in
conjunction with a RAP, {\bf throughput of more than $1$} is achievable (Figs. \ref{fig:upper_bound} and \ref{subfig:2lvlcompare}-\ref{subfig:k_approximation}), i.e., on
average more than one packet can be successfully decoded in each slot. Moreover, the proposed
strategy achieves a throughput close to double that of the relevant IRSA or CSA protocols, with just two power
levels. Of course, the power consumption with the proposed strategy is higher than CSA, however, since the system is interference limited, naively increasing the transmitted power would not yield any benefit.

To understand the benefit of increased power consumption, recall the main idea behind the improved throughput of IRSA \cite{liva} over ALOHA was to introduce repetition in transmission, thereby increasing the average power transmission and exploit the SIC capability. Thus, higher power consumption allowed higher throughput. 
CSA \cite{csa_paper} improved the power efficiency over IRSA by using more efficient codes compared to just repetition code in IRSA. 
To further exploit the SIC, as discussed before, and to decode more than one packet per slot, we need to create a power profile at the receiver where some packets are at much higher power level than the rest. The proposed strategy accomplishes this by using multiple power levels with sufficient multiplicative gaps between the levels, thus requiring larger power consumption, but allowing fundamental improvement in achievable throughputs.
\vspace{-0.2in}
\subsection{Our results} 
In this paper, we propose a multi-level random (with distribution $\Delta$) power transmit strategy 
which is used in conjunction with the RAP (with distribution $\Lambda$). With the transmit strategy, in the slot chosen according to distribution $\Lambda$, a packet is transmitted with power level $P \in {\cal P}$ chosen according to $\Delta$. The optimization problem we solve is to maximize the throughput as a function of $\Delta$ and $\Lambda$ for common RAPs, such as ALOHA, IRSA and CSA.
Our contributions are summarized as follows.
\begin{itemize}
\item For the case of ALOHA, we give an exact characterization of the throughput of the proposed strategy for two power levels, which can be directly optimized over $\Delta$.
\item With IRSA, an exact expression for throughput is not possible, however, using the expressions that are derived for iterative decoding techniques in prior work, we derive an expression for the probability of successful 
decoding of any packet asymptotically. The derived expressions significantly reduce the complexity of solving the optimization problem of maximizing the throughput over $\Delta$ and $\Lambda$. 
Similar analytical results are possible for CSA, but are omitted for brevity, 
since they do not bring any new ideas with it.
\item Since the achievable throughputs with IRSA as the RAP are not amenable to analytical expression, we derive upper bounds, that characterize fundamental limits on throughput with the proposed strategy. The derived bounds are shown to closely match the achievable throughputs via simulation. 
\item Extensive simulation results for achievable throughput are presented for the proposed strategy, with ALOHA/IRSA/CSA. We conclude that there is a fundamental improvement (close to double) in throughput with the proposed strategy at the cost of higher average power consumption. One main key observation is that {\bf throughput higher than one} is possible for a many appropriate choices of parameters, e.g. Figs. \ref{fig:upper_bound} and \ref{subfig:2lvlcompare}-\ref{subfig:k_approximation}, which is almost double  than possible for ALOHA/IRSA/CSA alone. Moreover, most of the throughput gain can be extracted via employing just two different power levels, and there is only mild incremental gain with more than two power levels. Thus, the complexity of practical implementation can be kept low by choosing only two power levels.

\item As a side result, we also analyze the throughput of the IRSA protocol under the path-loss channel model with a single power level,  which has escaped analytical tractability in the past. Towards this end, we map the IRSA protocol under the path-loss channel model without any power control to the IRSA with $n$-power levels under an ideal channel model. Leveraging results developed for analyzing the IRSA with $n$-power levels under an ideal channel model, we approximate the throughput achievable with IRSA protocol under the path-loss channel model with a single power level.
\end{itemize} 


\subsection{Other Related Work}
Random access protocols have been considered in variety of different contexts and not just maximizing the throughput. For example, an important metric is the stability of the system, that defines the largest packet arrival rates at nodes, such that the sum of the expected queue lengths across different nodes remains bounded. Extensive work has been reported in studying the stability properties of slotted ALOHA protocol \cite{szpankowski1994stability, ephremides1998information, rao1988stability, luo1999stability}. Another interesting direction has been to understand the information theoretic limits of random access protocols as initiated in \cite{massey1985collision}, where the nodes may not even be slot synchronized, which was later extended in \cite{hui1984multiple, thomas2000capacity, chen2017capacity}. 

For the throughput problem, extensions of the CSA protocol have been proposed in \cite{sun2017coded} for the erasure channel,  with finite blocklength \cite{lazaro2017finite, dovelos2017finite,  i2018finite}, with multiple parallel links for each slot that do not interfere with each other \cite{stefanovic2017asymptotic}. For the basics of iterated decoding of slotted ALOHA we refer the reader to \cite{narayanan2012iterative}.

During the course of writing the paper, we found that just the raw idea of using multiple power levels chosen randomly with random access protocols can be found in a two-page short note \cite{bandai2017power}, however, without any analysis or simulation results.


\begin{figure}[H]
	\begin{subfigure}[b]{0.5\textwidth}
	\centering
	\begin{tikzpicture}[scale = 0.7]
		% Basic Grid for the matrix
		\foreach \x in {0,...,-3}
		\draw[dashed] (0,\x) -- (8,\x);
		\foreach \x in {0,2,4,6,8}
		\draw[dashed] (\x,0) -- (\x,-3);
		\foreach \x in {1,2,3,4}
		\node at (2*\x-1,0.3) {Slot \x};
		\foreach \x in {1,2,3}
		\node at (-0.8, -\x + 0.5) {User \x};
		% Putting blocks for user 1
		\foreach \x in {1,2,3,4}
		\node [draw, fill= gray!30, shape=rectangle, minimum width=1cm, minimum
        height=0.5cm, anchor=center, rounded corners] at (2*\x-1,-0.5) {$P =
        1$};
		\foreach \x in {2,4}
		\node [draw, fill= gray!30, shape=rectangle, minimum width=1cm, minimum
        height=0.5cm, anchor=center, rounded corners] at (2*\x-1,-1.5) {$P =
        1$};
		\foreach \x in {2,4}
		\node [draw, fill= gray!30, shape=rectangle, minimum width=1cm, minimum
        height=0.5cm, anchor=center, rounded corners] at (2*\x-1,-2.5) {$P =
        1$};
	\end{tikzpicture}
	\caption{}
	\end{subfigure}
	\begin{subfigure}[b]{0.5\textwidth}
	\centering
	\begin{tikzpicture}[scale = 0.7]
		\node[draw, shape = rectangle, anchor = center, minimum width = 0.5cm,
		minimum height = 0.5cm] at (0,2.5) (s1) {};
		\node[draw, shape = rectangle, anchor = center, minimum width = 0.5cm, minimum
			height = 0.5cm] at (2,2.5) (s3) {};
		\node[draw, shape = rectangle, anchor = center, minimum width = 0.5cm,
		minimum height = 0.5cm] at (4,2.5) (s4) {};
		\node[draw, shape = rectangle, anchor = center, minimum width = 0.5cm, minimum
			height = 0.5cm] at (6,2.5) (s5) {};
		\node[draw, shape = circle, anchor = center, minimum width = 0.5cm, minimum height = 0.5cm] at (1.5,0.5) (u1) {};
		\node[draw, shape = circle, anchor = center, minimum width = 0.5cm, minimum height = 0.5cm] at (3,0.5) (u2) {};
		\node[draw, shape = circle, anchor = center, minimum width = 0.5cm, minimum height = 0.5cm] at (4.5,0.5) (u3) {};
		\draw (u1.north) -- (s1.south);
		\draw (u1.north) -- (s3.south);
		\draw (u1.north) -- (s4.south);
		\draw (u1.north) -- (s5.south);
		\draw (u2.north) -- (s3.south);
		\draw (u2.north) -- (s5.south);
		\draw (u3.north) -- (s3.south);
		\draw (u3.north) -- (s5.south);
		\foreach \x in {1,2,3,4}
		\node at (2*\x- 2,3) {$s_\x$};
		\foreach \x in {1,2,3}
		\node at (1.5*\x,0) {$u_\x$};
	\end{tikzpicture}
	\caption{}
	\end{subfigure}
	\caption{(a) denotes a MAC frame with 3 users and 4 slots where each user
	employs a repetition code independently and uses the same power $P = 1$, 
	(b) denotes the bipartite graph representation of the same.}
	\label{fig:irsa_slots_rep}
\end{figure}

\begin{figure}[H]
	\begin{subfigure}[b]{0.5\textwidth}
	\centering
	\begin{tikzpicture}[scale = 0.5]
		\node[draw, shape = rectangle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm,  fill = gray!40] at (0,2.5) (s1) {};
		\node[draw, shape = rectangle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm, ] at (2,2.5) (s3) {};
		\node[draw, shape = rectangle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm, ] at (4,2.5) (s4) {};
		\node[draw, shape = rectangle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm, ] at (6,2.5) (s5) {};
		\node[draw, shape = circle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm, fill = gray!40] at (1.5,0.5) (u1) {};
		\node[draw, shape = circle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm,] at (3,0.5) (u2) {};
		\node[draw, shape = circle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm,] at (4.5,0.5) (u3) {};
		\draw[dotted] (u1.north) -- (s1.south);
		\draw[dashed] (u1.north) -- (s3.south);
		\draw[dotted] (u1.north) -- (s4.south);
		\draw[dashed] (u1.north) -- (s5.south);
		\draw[] (u2.north) -- (s3.south);
		\draw[] (u2.north) -- (s5.south);
		\draw[] (u3.north) -- (s3.south);
		\draw[] (u3.north) -- (s5.south);
	\end{tikzpicture}
	\caption{Iteration 1}
	\end{subfigure}
	\begin{subfigure}[b]{0.5\textwidth}
	\centering
	\begin{tikzpicture}[scale = 0.5]
		\node[draw, shape = rectangle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm,  fill = gray!40] at (0,2.5) (s1) {};
		\node[draw, shape = rectangle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm, ] at (2,2.5) (s3) {};
		\node[draw, shape = rectangle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm, ] at (4,2.5) (s4) {};
		\node[draw, shape = rectangle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm, ] at (6,2.5) (s5) {};
		\node[draw, shape = circle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm, fill = gray!40] at (1.5,0.5) (u1) {};
		\node[draw, shape = circle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm,] at (3,0.5) (u2) {};
		\node[draw, shape = circle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm,] at (4.5,0.5) (u3) {};
		%\draw[dotted] (u1.north) -- (s1.south);
		%\draw[dashed] (u1.north) -- (s3.south);
		%\draw[dashed] (u1.north) -- (s4.south);
		%\draw[dashed] (u1.north) -- (s5.south);
		\draw[] (u2.north) -- (s3.south);
		\draw[] (u2.north) -- (s5.south);
		\draw[] (u3.north) -- (s3.south);
		\draw[] (u3.north) -- (s5.south);
	\end{tikzpicture}
	\caption{Iteration 2}
	\end{subfigure}
	\caption{Graphical representation of the decoding process}
	\label{fig:irsa_decoding_rep}
\end{figure}
\vspace{-0.4in}
\begin{figure}[H]
	\begin{subfigure}[b]{0.5\textwidth}
	\centering
	\begin{tikzpicture}[scale = 0.7]
		% Basic Grid for the matrix
		\foreach \x in {0,...,-3}
		\draw[dashed] (0,\x) -- (8,\x);
		\foreach \x in {0,2,4,6,8}
		\draw[dashed] (\x,0) -- (\x,-3);
		\foreach \x in {1,2,3,4}
		\node at (2*\x-1,0.3) {Slot \x};
		\foreach \x in {1,2,3}
		\node at (-0.8, -\x + 0.5) {User \x};
		% Putting blocks for user 1
		\foreach \x in {1,4}
		\node [draw, fill= gray!30, shape=rectangle, minimum width=1cm, minimum
		height=0.5cm, anchor=center, rounded corners] at (2*\x-1,-0.5) {$P =
		1$};
		\foreach \x in {2,3}
		\node [draw, fill= gray!30, shape=rectangle, minimum width=1cm, minimum
		height=0.5cm, anchor=center, rounded corners] at (2*\x-1,-0.5) {$P =
		4$};
		\foreach \x in {2}
		\node [draw, fill= gray!30, shape=rectangle, minimum width=1cm, minimum
		height=0.5cm, anchor=center, rounded corners] at (2*\x-1,-1.5) {$P =
		4$};
		\foreach \x in {4}
		\node [draw, fill= gray!30, shape=rectangle, minimum width=1cm, minimum
		height=0.5cm, anchor=center, rounded corners] at (2*\x-1,-1.5) {$P =
		1$};
		\foreach \x in {2,4}
		\node [draw, fill= gray!30, shape=rectangle, minimum width=1cm, minimum
		height=0.5cm, anchor=center, rounded corners] at (2*\x-1,-2.5) {$P =
		1$};
	\end{tikzpicture}
	\caption{}
	\end{subfigure}
	\begin{subfigure}[b]{0.5\textwidth}
	\centering
	\begin{tikzpicture}[scale = 0.7]
		\node[draw, shape = rectangle, anchor = center, minimum width = 0.5cm,
		minimum height = 0.5cm] at (0,2.5) (s1) {};
		\node[draw, shape = rectangle, anchor = center, minimum width = 0.5cm, minimum
			height = 0.5cm] at (2,2.5) (s3) {};
		\node[draw, shape = rectangle, anchor = center, minimum width = 0.5cm,
		minimum height = 0.5cm] at (4,2.5) (s4) {};
		\node[draw, shape = rectangle, anchor = center, minimum width = 0.5cm, minimum
			height = 0.5cm] at (6,2.5) (s5) {};
		\node[draw, shape = circle, anchor = center, minimum width = 0.5cm, minimum height = 0.5cm] at (1.5,0.5) (u1) {};
		\node[draw, shape = circle, anchor = center, minimum width = 0.5cm, minimum height = 0.5cm] at (3,0.5) (u2) {};
		\node[draw, shape = circle, anchor = center, minimum width = 0.5cm, minimum height = 0.5cm] at (4.5,0.5) (u3) {};
		\draw (u1.north) -- (s1.south);
		\draw (u1.north) -- (s3.south);
		\draw (u1.north) -- (s4.south);
		\draw (u1.north) -- (s5.south);
		\draw (u2.north) -- (s3.south);
		\draw (u2.north) -- (s5.south);
		\draw (u3.north) -- (s3.south);
		\draw (u3.north) -- (s5.south);
		\foreach \x in {1,2,3,4}
		\node at (2*\x- 2,3) {$s_\x$};
		\foreach \x in {1,2,3}
		\node at (1.5*\x,0) {$u_\x$};
	\end{tikzpicture}
	\caption{}
	\end{subfigure}
	\caption{(a) denotes a MAC frame with 3 users and 4 slots where each user
	employs a repetition code independently and also employ power control by
	transmitting packets at different power levels chosen independently for the
	set $\mathcal{P} = \{1,4\}$,
	(b) denotes the bipartite graph representation of the same.}
	\label{fig:irsa_pc_slots_rep}
\end{figure}

\begin{figure}[H]
	\begin{subfigure}[b]{0.32\textwidth}
	\centering
	\begin{tikzpicture}[scale = 0.6]
		\node[draw, shape = rectangle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm,  fill = gray!40] at (0,2.5) (s1) {};
		\node[draw, shape = rectangle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm, ] at (2,2.5) (s3) {};
		\node[draw, shape = rectangle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm, fill = gray!40 ] at (4,2.5) (s4) {};
		\node[draw, shape = rectangle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm, ] at (6,2.5) (s5) {};
		\node[draw, shape = circle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm, fill = gray!40] at (1.5,0.5) (u1) {};
		\node[draw, shape = circle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm,] at (3,0.5) (u2) {};
		\node[draw, shape = circle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm,] at (4.5,0.5) (u3) {};
		\draw[dotted] (u1.north) -- (s1.south);
		\draw[dashed] (u1.north) -- (s3.south);
		\draw[dotted] (u1.north) -- (s4.south);
		\draw[dashed] (u1.north) -- (s5.south);
		\draw[] (u2.north) -- (s3.south);
		\draw[] (u2.north) -- (s5.south);
		\draw[] (u3.north) -- (s3.south);
		\draw[] (u3.north) -- (s5.south);
	\end{tikzpicture}
	\caption{Iteration 1}
	\end{subfigure}
	\begin{subfigure}[b]{0.32\textwidth}
	\centering
	\begin{tikzpicture}[scale = 0.6]
		\node[draw, shape = rectangle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm,  fill = gray!40] at (0,2.5) (s1) {};
		\node[draw, shape = rectangle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm, fill = gray!40] at (2,2.5) (s3) {};
		\node[draw, shape = rectangle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm, fill = gray!40] at (4,2.5) (s4) {};
		\node[draw, shape = rectangle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm, ] at (6,2.5) (s5) {};
		\node[draw, shape = circle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm, fill = gray!40] at (1.5,0.5) (u1) {};
		\node[draw, shape = circle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm, fill = gray!40] at (3,0.5) (u2) {};
		\node[draw, shape = circle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm,] at (4.5,0.5) (u3) {};
		%\draw[dotted] (u1.north) -- (s1.south);
		%\draw[dashed] (u1.north) -- (s3.south);
		%\draw[dashed] (u1.north) -- (s4.south);
		%\draw[dashed] (u1.north) -- (s5.south);
		\draw[dotted] (u2.north) -- (s3.south);
		\draw[dashed] (u2.north) -- (s5.south);
		\draw[] (u3.north) -- (s3.south);
		\draw[] (u3.north) -- (s5.south);
	\end{tikzpicture}
	\caption{Iteration 2}
	\end{subfigure}
	\begin{subfigure}[b]{0.32\textwidth}
	\centering
	\begin{tikzpicture}[scale = 0.6]
		\node[draw, shape = rectangle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm,  fill = gray!40] at (0,2.5) (s1) {};
		\node[draw, shape = rectangle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm, fill = gray!40] at (2,2.5) (s3) {};
		\node[draw, shape = rectangle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm, fill = gray!40] at (4,2.5) (s4) {};
		\node[draw, shape = rectangle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm, fill = gray!40] at (6,2.5) (s5) {};
		\node[draw, shape = circle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm, fill = gray!40] at (1.5,0.5) (u1) {};
		\node[draw, shape = circle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm, fill = gray!40] at (3,0.5) (u2) {};
		\node[draw, shape = circle, anchor = center, minimum width = 0.3cm,
		minimum height = 0.3cm,fill = gray!40] at (4.5,0.5) (u3) {};
		%\draw[dotted] (u1.north) -- (s1.south);
		%\draw[dashed] (u1.north) -- (s3.south);
		%\draw[dashed] (u1.north) -- (s4.south);
		%\draw[dashed] (u1.north) -- (s5.south);
		%\draw[dotted] (u2.north) -- (s3.south);
		%\draw[dashed] (u2.north) -- (s5.south);
		\draw[dotted] (u3.north) -- (s3.south);
		\draw[dotted] (u3.north) -- (s5.south);
	\end{tikzpicture}
	\caption{Iteration 3}
	\end{subfigure}
	\caption{Graphical representation of the decoding process}
	\label{fig:irsa_decoding_rep}
\end{figure}

\begin{comment}
\begin{figure}[H]
\minipage{0.333\textwidth}
  \includegraphics[width=\linewidth]{plots/intro_sa_sa_dpc}
  \label{fig:intro_sa_sa_dpc}
\endminipage\hfill
\minipage{0.333\textwidth}
  \includegraphics[width=\linewidth]{plots/intro_irsa_irsa_pc}
  \label{fig:intro_irsa_irsa_pc}
\endminipage\hfill
\minipage{0.333\textwidth}%
  \includegraphics[width=\linewidth]{plots/intro_csa_csa_pc}
  \label{fig:intro_csa_csa_pc}
\endminipage
\caption{Option 1}
\end{figure}
\end{comment}

\begin{figure}[H]
\minipage{0.55\textwidth}
  \includegraphics[width=\linewidth]{plots/intro_irsa_irsa_pc}
  \label{fig:intro_irsa_irsa_pc}
\endminipage\hfill
\minipage{0.55\textwidth}
  \includegraphics[width=\linewidth]{plots/intro_csa_csa_pc}
  \label{fig:intro_csa_csa_pc}
\endminipage
\caption{$P$ is the minimum power required to ensure successful decoding at the
base station and $P_{avg}$ refers to ther average energy consumption per frame.}
\label{fig:intro_comparison}
\end{figure}

\begin{comment}
\begin{figure}[H]
\minipage{0.55\textwidth}
  \includegraphics[width=\linewidth]{plots/intro_sa_irsa_irsa_pc}
  \label{fig:intro_sa_irsa_irsa_pc}
\endminipage\hfill
\minipage{0.55\textwidth}
  \includegraphics[width=\linewidth]{plots/intro_csa__liva_csa_pc}
  \label{fig:intro_sa_csa_csa_pc}
\endminipage
\caption{ \textcolor{blue}{YYY Note to Rahul : Plot with CSA data taken directly
from the Liva's paper and plotted only uptil 1}}
\end{figure}
\end{comment}


